Probabilistic Conceptual Explainers: Trustworthy Conceptual Explanations for Vision Foundation Models

Vision transformers (ViTs) have emerged as a significant area of focus, particularly for their capacity to be jointly trained with large language models and to serve as robust vision foundation models. Yet, the development of trustworthy explanation methods for ViTs has lagged, particularly in the context of post-hoc interpretations of ViT predictions. Existing sub-image selection approaches, such as feature-attribution and conceptual models, fall short in this regard. This paper proposes five desiderata for explaining ViTs -- faithfulness, stability, sparsity, multi-level structure, and parsimony -- and demonstrates the inadequacy of current methods in meeting these criteria comprehensively. We introduce a variational Bayesian explanation framework, dubbed ProbAbilistic Concept Explainers (PACE), which models the distributions of patch embeddings to provide trustworthy post-hoc conceptual explanations. Our qualitative analysis reveals the distributions of patch-level concepts, elucidating the effectiveness of ViTs by modeling the joint distribution of patch embeddings and ViT's predictions. Moreover, these patch-level explanations bridge the gap between image-level and dataset-level explanations, thus completing the multi-level structure of PACE. Through extensive experiments on both synthetic and real-world datasets, we demonstrate that PACE surpasses state-of-the-art methods in terms of the defined desiderata.

==> sec/0_abstract.tex <==
\begin{abstract}
% Vision transformers (ViTs) have garnered significant attention, especially with its advantage of joint training with large language models. However, reliable explanation methods for ViTs have received much less attention. Specifically, existing sub-image selection paradigms, including feature-attribution and conceptual models, are not sufficient to be well adapted into post-hoc interpretations of ViT predictions. In this paper, we first propose five desiderata for explaining ViTs - faithfulness, stability, sparsity, multi-level structure, and parsimony - and show that existing methods do not satisfy them. We then propose a simple and straightforward variational Bayesian explanation framework, dubbed TRUstworthy Conceptual Explanations (TRUCE), to model the distributions of patch embeddings and provide trustworthy conceptual explanations. Furthermore, we unveil the profound semantics hidden in the patch representations inside ViTs, and show that image patches are intrinsically well-posed sub-image level for conceptual interpretations. Experiments across various datasets show that our TRUCE (1) outperform state-of-the-art on the defined properties across synthetic and real-world datasets. (2) well aligns with human intuitive in the qualitative study, which is demonstrated by the fine-grained labeled concepts.

Vision transformers (ViTs) have emerged as a significant area of focus, particularly for their capacity to be jointly trained with large language models. Yet, the development of trustworthy explanation methods for ViTs has lagged, particularly in the context of post-hoc interpretations of ViT predictions. Existing sub-image selection approaches, such as feature-attribution and conceptual models, fall short in this regard. This paper proposes five desiderata for explaining ViTs -- faithfulness, stability, sparsity, multi-level structure, and parsimony -- and demonstrates the inadequacy of current methods in meeting these criteria comprehensively. We introduce a variational Bayesian explanation framework, dubbed Variational Concept Explainers (VaCE), which models the distributions of patch embeddings to provide trustworthy post-hoc conceptual explanations. 
Our qualitative analysis reveals the distributions of patch-level concepts, elucidating the effectiveness of ViTs by modeling the joint distribution of patch embeddings and ViT's predictions. Moreover, these patch-level explanations bridge the gap between image-level and dataset-level explanations, thus completing the multi-level structure of VaCE. 
Through extensive experiments on both synthetic and real-world datasets, we demonstrate that VaCE surpasses state-of-the-art methods in terms of the defined desiderata\footnote{{Code will soon be available at https://github.com/Wang-ML-Lab/VaCE}}. % , without the need for additional cropping and image segmentation
\end{abstract}

% , but also aligns closely with human intuition, as evidenced by qualitative studies involving finely labeled concepts.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Vision Transformers (ViTs)~\citep{dosovitskiy2020vit} and their variants~\citep{liu2021swin,touvron2021deit,radford2021clip} have emerged as pivotal models in computer vision, leveraging stacked self-attention blocks to encode raw inputs and produce patch-wise embeddings as contextual representations. Given their increasing application in high-risk domains such as autonomous driving, explainability has become a critical concern.


To date, post-hoc explanations in computer vision often involve attributing predictions to specific image regions. However, we identify two primary limitations in current methods: (1) {
Existing conceptual explanation methods~\cite{fel2023holistic,fel2023craft,ghorbani2019ace,zhang2021ice} are not fully compatible with transformer-based models like vision transformers (ViTs), and they also fall short in offering a cohesive structure for dataset-image-patch analysis of input images.}
%Existing conceptual explanation methods~\cite{fel2023craft,ghorbani2019ace,zhang2021ice} %either focus on identifying superpixels crucial for class prediction~\citep{ribeiro2016lime,lundberg2017shap,simonyan2013saliency}, or localizing the receptive field of convolution kernels linked to specific concepts~\cite{fel2023craft,ghorbani2019ace,zhang2021ice},. These \emph{sub-image selection paradigms}, however, do not seamlessly integrate with transformer-based models like ViTs, \red{nor do they 
%lag in offering a cohesive dataset-image-patch structure of the input images.} %Conversely, we unravel the cohesive dataset-image-patch structure of concepts from ViT patch embeddings using a hierarchical variational Bayes framework.}
%nor do they adequately provide high-quality conceptual explanations. Surprisingly, we discover that ViTs inherently position image patches at a sub-image level with significant visual semantics, allowing for a straightforward conceptual explanation model by modeling the distribution of these patches. 
(2) Current state-of-the-art methods~\citep{pan2021agi,fel2023craft,colin2022cannot} evaluate visual concepts through subjective human utility scores or limited quantitative analysis, lacking a fair and consistent comparison framework. To address this, we propose a systematic set of desiderata 
for post-hoc conceptual explanations 
for ViTs, namely (see formal definitions in~\secref{sec:concept_def}): 
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
\item \emph{Faithfulness:} The explanation should be faithful to the explained ViT and able to recover its prediction. 
\item \emph{Stability:} The explanation should be stable for different perturbed versions of the same image. 
\item \emph{Sparsity:} For each prediction's explanation, only a small subset of concepts are relevant. 
\item \emph{Multi-Level Structure:} There should be dataset-level, image-level, and patch-level explanations. 
\item \emph{Parsimony:} There are a small number of concepts in total {(see~\appref{app:sparse_vs_pars} for more details)}. 
\end{itemize}
% \emph{faithfulness, stability, sparsity, multi-level structure, and parsimony}. 
{While previous research~\cite{kim2018tcav,fel2023craft,oikarinen2023label, gilpin2018explaining, murdoch2019definitions} has proposed and met different dimensions of the learned concepts, these studies often lack a comprehensive evaluation. }%Consequently, existing methodologies may be inadequate for delivering trustworthy explanations.}
In this paper, we propose Variational Concept Explainers (VaCE) to provide trustworthy conceptual explanations aligned with these desiderata. For example, to enable \textbf{\emph{multi-level}} explanations, we 
(1) model $K$ concepts as a mixture of $K$ Gaussian patch-embedding distributions, 
(2) treat the explained ViT's patch-level embeddings as observed variables, 
% \red{and also take into account the predicted label during training to enhance \textbf{\emph{faithfulness}}} 
(3) learn a hierarchical Bayesian model that generates these embeddings in a top-down manner, from \emph{dataset-level} concepts through \emph{image-level} concepts to \emph{patch-level} embeddings, and (4) infer these multi-level concepts as our multi-level conceptual explanations; 
%To enhance \textbf{\emph{stability}}, our hierarchical Bayesian model ensures similarity between the concepts inferred from the original image and those from its perturbed versions.
to enhance \textbf{\emph{stability}}, our hierarchical Bayesian model ensures that the inferred concepts from two different perturbed versions of the same image remain similar to each other. 
Our contributions are: % as follows:
% itemize enumerate
%\begin{compactum}
\begin{enumerate}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    % \item We identify the limitations of existing sub-image selection paradigms in interpretation models and address this by treating image patches as natural sub-image-level representations. This approach allows us to model patch embeddings in the concept space, revealing profound multi-level semantics.
    \item We comprehensively study a systematic set of five desiderata \emph{faithfulness, stability, sparsity, multi-level structure}, and \emph{parsimony} when generating trustworthy concept-level explanations for ViTs. 
    \item We develop the first general method,  dubbed Variational Concept Explainers (VaCE), as a variational Bayesian framework that satisfies these desiderata. 
    \item Through both quantitative and qualitative evaluations, our method demonstrates superior performance in explaining post-hoc ViT predictions via visual concepts, outperforming state-of-the-art methods across various synthetic and real-world datasets.
\end{enumerate}




%end{compactum}







==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
